Aspect-augmented Adversarial Networks for Domain Adaptation

We introduce a neural method for transfer learning between two (source and target) classification tasks or aspects over the same domain. Rather than training on target labels, we use a few keywords pertaining to source and target aspects indicating sentence relevance instead of document class labels. Documents are encoded by learning to embed and softly select relevant sentences in an aspect-dependent manner. A shared classifier is trained on the source encoded documents and labels, and applied to target encoded documents. We ensure transfer through aspect-adversarial training so that encoded documents are, as sets, aspect-invariant. Experimental results demonstrate that our approach outperforms different baselines and model variants on two datasets, yielding an improvement of 27% on a pathology dataset and 5% on a review dataset.

==> intro.tex <==
%!TEX root = paper.tex
\section{Introduction}

Deep learning methods are highly effective when they can be trained with large amounts of labeled training data in the domain of interest. While such data are not always available in real applications, it is nevertheless often possible to find labeled data in another related domain or for another related task. Considerable effort has gone into designing domain transfer algorithms that leverage such related data~\cite{glorot2011domain,chen2012marginalized,zhou2016bi}. In a typical case, the related domain involves the same classification task (e.g., sentiment analysis) but over different types of examples (e.g., hotel vs restaurant reviews). Labeled training data are available only in the source domain (e.g., hotel reviews) while the task is to provide an effective method for the target domain (e.g., restaurant reviews) without any additional labeled examples. 


% \begin{figure}[t]
% \centering
% \includegraphics[width=0.46\textwidth]{figures/pathology.pdf}
% \caption{A snippet of a breast pathology report with diagnosis results for two types of disease. Evidence for both results is in red and blue, respectively. }\label{fig:pathology}
% \vspace{-0.1in}
% \end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{figures/task.pdf}
\caption{\add{Comparisons between (a) standard domain adaptation and (b) our aspect transfer problem. Note that in domain adaptation input documents are naturally \emph{different} for the two domains while in aspect transfer both aspects are in the \emph{same} example. The model must find the correct fragment for each aspect (marked by solid line for source and dash line for target) in order to succeed in aspect transfer.}
}\label{fig:pathology}
\vspace{-0.1in}
\end{figure}

In this paper we are primarily interested in transfer between two classification tasks over the same domain, i.e., over the same set of examples. We call this ``aspect transfer'' as the two classification tasks can be thought to pertain to different aspects of the same example. For example, the target goal may be to classify pathology reports (shown in Figure \ref{fig:pathology}b) for the presence of lymph invasion but the available training data involve only annotations for carcinoma in the same reports. \add{Figure \ref{fig:pathology} illustrates how aspect transfer is different from standard domain adaptation (DA). Both transfer problems have to solve the challenge in learning the correspondence of keyword information (in bold) between source and target domains or aspects. However, }existing DA methods do not directly solve this aspect transfer problem because input examples are the \emph{same} across the two aspects. \add{As a result, DA methods will always predict the same label for both aspects and thus fail. The model must learn to extract information from the correct fragment in order to succeed.} 

\add{To address this challenge, we propose to encode the document in an aspect-driven fashion.} Specifically, our approach builds on auxiliary aspect-relevance annotations of sentences which are considerably easier to obtain than actual class labels. Relevance merely indicates a possibility that the answer could be found in a sentence, not what the answer is. One can often write simple keyword rules that identify sentence relevance to a particular aspect through representative terms, e.g., specific hormonal markers in the context of pathology reports. 
%Similar keywords can also indicate absence of relevance.
We can also use keywords of other irrelevant aspects to indicate absence of relevance.
Annotations of this kind can be readily provided by domain experts, or extracted from medical literature such as codex rules in pathology~\cite{pantanowitz2008informatics}. We therefore assume a small number of relevance annotations pertaining to both source and target aspects as a form of weak supervision to learn a sentence-level aspect relevance. This aspect relevance permits us to learn how to encode the examples (e.g., pathology reports) from the point of view of the desired aspect. Specifically, in our approach we construct different aspect-dependent encodings of the same report by softly selecting aspect-relevant sentences from the report.

Our aspect-driven encoding reduces the aspect transfer problem closer to the realm of standard DA. The two domains as in standard DA are induced by different ways of interpreting the same example in our case. These interpretations are themselves learned based on relevance feedback, thus naturally pulled apart. We employ only one label classifier shared between the aspects but it is exercised differently due to aspect-driven encoding of examples. To ensure that the classifier can be adjusted only based on the source class labels and still reasonably applied to the target encodings, we must align the two sets of encoded examples. \add{Learning this alignment is possible in our case because certain common keywords are directly transferable and can serve as anchors of an invariant space. For example, in pathology reports ``identified'' indicates a positive label in both carcinoma and invasion aspects. The key challenge is to learn to project aspect-specific information to this invariant space.}

To address this challenge, we introduce an adversarial domain classifier analogously to recent successful use of adversarial training in computer vision~\cite{ganin2014unsupervised}. \add{This approach is motivated by the theory \cite{ben2007analysis,ben2010theory} that a good transferable representation is one that a classifier cannot learn to identify the origin domain of the input. In particular, the domain classifier is trained to predict the origin aspect/domain of the encoded document. It will achieve a high accuracy as long as encodings contain aspect-specific information. The key of adversarial training is to update the encoder as an adversary against the classifier. In other words, we reverse the gradient from the domain classifier (the adversary) therefore encouraging encodings that make the classifier fail. The encoder therefore learns to eliminate aspect-specific information, establishing aspect-invariance encodings. Such encodings will allow transfer across aspects.} 
Note that this invariance is enforced on the level of sets, not individual examples or reports; encoding of any specific report should remain substantially different for label prediction. To learn the invariance, All the three components in our approach, 1) aspect-driven encoding, 2) classification of source labels, and 3) domain adversary, are trained jointly (concurrently) to complement and balance each other.

%Our relevance driven encoding returns the aspect-transfer problem closer to the realm of standard domain adaption. We employ a shared end classifier between the tasks but it is exercised differently due to aspect-driven encoding of examples. The two domains in a standard domain adaption are therefore induced in our case by different ways of interpreting the same examples. Note that these interpretations are themselves learned based on relevance feedback, thus naturally pulled apart. To ensure that the classifier can be adjusted only based on the source class labels and also reasonably applies to the target encodings, we must align the two sets of encoded examples. This alignment or invariance is enforced on the level of sets, not individual examples or reports; aspect-drive encoding of any specific report should remain substantially different for the two tasks since the encoded examples are passed on to the same classifier. To learn the invariance, we introduce an adversarial domain classifier analogously to recent successful use of adversarial training in computer vision~\cite{ganin2014unsupervised}. The role of the adversary is to learn to distinguish between the two types of encodings, establishing invariance (as sets) when it fails. All the three components in our approach, 1) aspect-driven encoding, 2) classification of source labels, and 3) domain adversary, are trained jointly (concurrently) to complement and balance each other.

Adversarial training of domain and label classifiers can be challenging to stabilize. In our setting, sentences are encoded with a shared convolutional model, weighted by predicted aspect relevance, and then combined into aspect-driven document representations. Feedback from adversarial training can be an unstable guide for how the sentences should be encoded in the first place. To this end, we incorporate an additional word-level autoencoder reconstruction loss to ground the convolutional processing of sentences. We empirically demonstrate that this additional objective yields richer and more diversified feature representations, improving transfer. 

We evaluate our approach on pathology reports (aspect transfer) as well as on a more standard review dataset (domain adaptation). On the pathology dataset, we explore cross-aspect transfer across different types of breast disease. Specifically, we test on six adaptation tasks, consistently outperforming all other baselines. Overall, our full model achieves 27\% and 20.2\% absolute improvement arising from aspect-driven encoding and adversarial training, respectively. Moreover, our unsupervised adaptation method is only 5.7\% behind the accuracy of a supervised target model. On the review dataset, we test adaptation from hotel to restaurant reviews.
Our model outperforms the marginalized denoising autoencoder~\cite{chen2012marginalized} by 5\%.
%Our model outperforms the baseline without adversarial training by 2.5\%. 
Finally, we examine and illustrate the impact of individual components on the resulting performance. 


%We evaluate our approach on pathology reports (aspect transfer) as well as on more standard review dataset (domain adaptation). On the pathology dataset, we explore cross-aspect transfer across different types of breast disease. Specifically, we test on six adaptation tasks, consistently outperforming all other baselines. Overall, our full model achieves 12.8\% absolute improvement arising from adversarial training. Moreover, our unsupervised adaptation method is only 2.8\% behind the accuracy of a supervised target model. On the review dataset, we test adaptation from hotel to restaurant reviews. Our model achieves the best performance on four out of five adaptation tasks, and outperforms the baseline without adversarial training by 2.5\%. Finally, we examine and illustrate the impact of individual components on the resulting performance.  

%This document encoding mechanism brings the problem closer to the realm of standard domain adaption. Such aspect-dependent encodings can be considered as features extracted from source or target domains, which are then passed to one label classifier that are shared between the two domains. To ensure that the classifier can be adjusted only based on the source class labels and also reasonably applies to the target encodings, we must align the two sets of encoded examples.\footnote{This alignment or invariance is enforced on the level of sets, not individual examples or reports; aspect-drive encoding of any specific report should remain substantially different for the two tasks since the encoded examples are passed on to the same classifier.}  Learning this alignment is possible because, as discussed above, some keywords are directly transferable and can serve as anchors for constructing this invariant space. To learn this invariant representation, we employ domain adversarial training analogously to recent success in computer vision~\cite{ganin2014unsupervised}. The core idea is to jointly learn a domain classifier (adversary) whose role is to distinguish between the two types of encodings. During training the encoder is updated with an adversarial objective to fail the classifier. The encoder therefore learns to eliminate aspect-specific information so that encodings look invariant (as sets) to the classifier, thus enabling transfer. All the three components in our approach, 1) aspect-driven encoding, 2) classification of source labels, and 3) domain adversary, are trained jointly (concurrently) to complement and balance each other.

==> introv0.tex <==
\section{Introduction}

The accuracy of deep learning methods depends on the access to large amounts of in-domain training data. While for many applications, such data is not available, it is often possible to find labeled data in another related domain. In this paper, we propose a transfer method for neural models that can utilize annotations developed for related domains and related tasks to improve performance in the target domain. 
% Yuan: saying "in the same domain" will cause confusion later, perhaps "in the same (set of) document(s)"
While cross-domain adaptation has been commonly considered in the literature, we are particularly interested in applying this method to transfer across aspects within the same domain. For example, when learning to classify pathology reports (shown in Figure \ref{fig:pathology}) for the presence of lymph invasion, we would like to utilize training data available for identifying carcinoma in the same report. %Figure \ref{fig:pathology} illustrates a breast %pathology report along with diagnosis results for two aspects %related to types of breast disease. If the model aims to %predict the label for lymphatic vessel invasion (LVI), it %should learn to extract features only from the second sentence %(in blue).

Existing domain adaptation approaches cannot be effectively applied for this task. For instance, one commonly used approach employs autoencoders to learn cross-domain representation so that a classifier trained on this representation can handle both source and target domains~\cite{glorot2011domain,chen2012marginalized,chopra2013dlid}. These methods learn representation without the awareness of different aspects in a document. In the case of aspect transfer, however, both aspects have to be predicted from the same document. As a result, both classifiers operate over the same representation from the very beginning, and will always predict the same label for both aspects. Moreover, since auotoencoders learn the representation in the task agnostic scenario, it is unlikely to be useful in this scenario. 

\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{figures/pathology.pdf}
\caption{A snippet of a breast pathology report with diagnosis results for two types of disease. Evidence for both results is in red and blue, respectively. }\label{fig:pathology}
\end{figure}

In this paper, we propose a novel approach that aims to find a balance between (1) learning an invariant representation that supports generalization across tasks and domains (2) tailoring the representation to a specific target task at the same time. We implement our model as an aspect-augmented adversarial network, building on successful use of these networks in computer vision~\cite{ganin2014unsupervised}. Our model is composed of an aspect-specific label predictor, a document encoder that extracts hidden features, and a domain classifier trained to predict the domain of the input document based on learned representation. The performance of this classifier naturally provides an effective measurement on cross-aspect dissimilarities. In other words, the domain classifier will perform poorly if features are aspect-invariant. We therefore jointly optimize the encoder as an adversary to promote features that fail the classifier, while also aiming to minimize the loss of the label predictor. 

% Yuan: the original paragraph is confusing because the keywords sound like the supervision for the label prediction rather than for the relevance scorer. I put the old version in old-intro.tex

%We are interested in employing this method for scenarios where label annotations are only available for the source aspect. However, to enable aspect transfer, we do require extra supervision to distinguish different aspects in the same document. As an alternative source of weak supervision, we assume a small set of keywords associated with each aspect, such as terms representative of a specific hormonal marker in a pathology report. Such annotations can be easily provided by domain experts, or extracted from medical literature such as codex rules in pathology. Our model utilizes these keywords by augmenting the document encoder with a sentence-level aspect-relevance scorer similar to the attention mechanism. These scores allow the model to selectively consider information from relevant fragments while ignoring the rest.

To enable aspect-specific transfer and classification, we augment the document encoder with a sentence-level aspect-relevance scorer similar to the attention mechanism. These scores allow the model to selectively consider information from relevant fragments while ignoring the rest. While we are interested in scenarios where annotations are only available for the source aspect, we do require supervision for training the relevance scorer to distinguish different aspects. As an alternative source of weak supervision, we assume a small set of keywords associated with each aspect, such as terms representative of a specific hormonal marker in a pathology report. Such annotations can be easily provided by domain experts, or extracted from medical literature such as codex rules in pathology.  

Another departure of our method from prior work relates to the use of reconstruction loss to stabilize adversarial training. Our initial experiments with the adversarial training revealed that the encoder tends to induce sparse and low-variance representations regardless of inputs, which in turn degrades prediction performance. To address this issue, we revisit the idea of autoencoders and introduce a word-level reconstruction loss that is jointly optimized with other components of the model. We empirically demonstrate that this new objective yields richer and more diversified feature representation, as reflected in improved adaptation performance.

We evaluate our model on a pathology report dataset and a review dataset. On the pathology dataset, we explore the task of cross-aspect adaptation across different types of breast disease. Specifically, we test on six adaptation tasks, and empirical results show that our method consistently outperforms all other baselines. We demonstrate that both adversarial training and aspect-relevance scoring play a crucial role in this task, yielding a 13\% and a 24\% absolute gain over the counterpart baseline respectively. Moreover, our unsupervised adaptation result is only 2.8\% behind the accuracy of a supervised model. On the review dataset, we test on adaptation from the hotel domain to the restaurant domain. Our model outperforms the no-adversarial-training baseline by 2.5\%. Finally, we analyze the behavior of adversarial training and assess the impact of individual components to the overall model performance.



==> new-intro2.tex <==
This document encoding mechanism brings the problem closer to the realm of standard domain adaption. Such aspect-dependent encodings can be considered as features extracted from source or target domains, which are then passed to a single label classifier that are shared between the two domains. To ensure that the classifier can be adjusted only based on the source class labels and also reasonably applies to the target encodings, we must align the two sets of encoded examples.\footnote{This alignment or invariance is enforced on the level of sets, not individual examples or reports; aspect-drive encoding of any specific report should remain substantially different for the two tasks since the encoded examples are passed on to the same classifier.}  Learning this alignment is possible because, as discussed above, some keywords are directly transferable and can serve as anchors for constructing this invariant space. To learn this invariant representation, we employ domain adversarial training analogously to recent success in computer vision~\cite{ganin2014unsupervised}. The core idea is to jointly learn a domain classifier (adversary) whose role is to distinguish between the two types of encodings. During training we update the encoder with an adversarial objective to fail the classifier. The encoder therefore learns to eliminate aspect-specific information so that encodings look invariant (as sets) to the classifier, thus enabling transfer. All the three components in our approach, 1) aspect-driven encoding, 2) classification of source labels, and 3) domain adversary, are trained jointly (concurrently) to complement and balance each other.

Adversarial training of domain and label classifiers can be challenging to stabilize. In our setting, feedback from adversarial training can be an unstable guide for how documents should be encoded. To address this issue, we incorporate an additional word-level autoencoder reconstruction loss to ground the convolutional processing of sentences. We empirically demonstrate that this additional objective yields richer and more diversified feature representations, improving transfer. 


==> old-intro.tex <==
One common deep learning approach for domain adaptation is to simply train a single autoencoder on texts from both the source and the target domains. A label predictor (e.g. SVM) is then trained on hidden representations induced by the autoencoder in a separate step \cite{glorot2011domain,chen2012marginalized,chopra2013dlid}. We argue that there are two main disadvantages of this autoencoder approach. First, this approach still provides no effective means to encourage the emergence of domain-invariant features.  Second, many classification tasks require attention to a particular aspect in texts while prior methods only predict the category based on an \emph{overall} representation of the input. Figure \ref{fig:pathology} illustrates a breast pathology report along with diagnosis results for two aspects related to types of breast disease. If the model aims to predict the label for lymphatic vessel invasion (LVI), it should learn to extract features only from the second sentence (in blue). Moreover, an autoencoder only learns task-independent feature representations which may not be optimal for the targeting classification task.
%Indeed, distilling domain-invariant properties have been shown to be the key to improving domain adaptation performance in the context of shallow learning \cite{}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The accuracy of deep learning methods depends on the access to large amounts of in-domain training data. While for many applications, such data is not available, it is often possible to find related data. In this paper, we propose a transfer method for neural models that can utilize annotations developed for related domains and related tasks. 
% Yuan: saying "in the same domain" will cause confusion later
While cross-domain adoptation has been commonly considered in the literature, we are particularly interested in applying this method to transfer across aspects within the same domain. For example, when learning to classify pathology reports (shown in Figure \ref{fig:pathology}) for the presence of lymph invasion, we would like to utilize training data available for identifying carcinoma in the same report. %Figure \ref{fig:pathology} illustrates a breast %pathology report along with diagnosis results for two aspects %related to types of breast disease. If the model aims to %predict the label for lymphatic vessel invasion (LVI), it %should learn to extract features only from the second sentence %(in blue).

Existing domain adaptation approaches cannot be effectively applied for this task. For instance, one commonly used approach employs autoencoders to learn cross-domain representation so that a classifier trained on this representation can handle both source and target domains~\cite{glorot2011domain,chen2012marginalized,chopra2013dlid}. However, in the case of aspect transfer, both aspects have to predicted from the same document, so both classifiers operate over the same representation from the very beginning. Moreover, since auotoencoders learn the representation in the task agnostic scenario, it is unlikely to be useful in this scenario. 

\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{figures/pathology.pdf}
\caption{A snippet of a breast pathology report with diagnosis results for two types of disease. Evidence for both results is in red and blue, respectively. }\label{fig:pathology}
\end{figure}

In this paper, we propose a novel approach that aims to find a balance between learning an invariant representation that supports generalization across tasks and domains, while at the same time is tailored to a specific target task. We implement our model as an aspect-augmented adversarial network, building on successful use of these networks in computer vision~\cite{ganin2014unsupervised}. Our model is composed of aspect-specific label predictors, a document encoder that extracts hidden features, and a domain classifier trained to predict the domain of the input document based on learned representation. The performance of this classifier naturally provides an effective measurement on cross-aspect dissimilarities. In other words, the domain classifier will perform poorly if features are aspect-invariant. We therefore jointly optimize the encoder as an adversary to promote features that fail the classifier, while also
aiming to minimize the loss of the label predictor. 

We are interested to employ this method for scenarios where the annotated data is only available for the source aspect. As an alternative source of weak supervision, we assume a small set of keywords associated with a target aspect, such as terms representative of a specific hormonal marker in a pathology report. Such annotations can be easily provided by domain experts, or extracted from medical literature such as codex rules in pathology. Our model utilizes this keywords, by augmenting the document encoder with a sentence-level aspect-relevance scorer similar to the attention mechanism. These scores allow the model to selectively consider information from relevant fragments while ignore the rest.

Another departure of our method relates to the use of reconstruction loss to stabilize adversarial 
training. Our initial experiments with the adversarial training revealed that the encoder tends to induce sparse and low-variance representations regardless of inputs, which in turn degrades prediction performance. To address this issue, we revisit the idea of autoencoders and introduce a word-level reconstruction loss that is jointly optimized with other components of the model. We empirically demonstrate that this new objective yields richer and more diversified feature representation, as reflected in improved adaptation performance.

We evaluate out model on a pathology reports dataset and a review dataset. On the pathology dataset, we explore the task of cross-aspect adaptation across different types of breast disease. Specifically, we test on six adaptation tasks, and empirical results show that our method consistently outperforms all other baselines. On average, our full model achieves 22.5\% absolute improvement over the counterpart without adversarial training. Moreover, our unsupervised adaptation result is only 2.6\% behind the accuracy of a supervised model. On the review dataset, we test on adaptation from the hotel domain to the restaurant domain. Our model achieves the best performance on four out of five adaptation tasks, and outperforms the no-adversarial-training baseline by 3.2\%. Finally, we analyze the behavior of adversarial training and assess the impact of individual components to the overall model performance.

==> old-related.tex <==
% domain adaptation, SCL etc. deep learning approach
% technically similar
% semeval shared task
% rationale augmented CNN
% In both approaches, the actual classifier/predictor is learned in a separate step using the feature representation learned by autoencoder(s)

\section{Related Work}

\paragraph{Domain Adaptation for Text Classification}
A large number of domain adaptation methods have been proposed in the context of shallow learning, ranging from data reweighing \cite{huang2006correcting,gong2013connecting} to learning correspondence between features \cite{blitzer2006domain,daume2009frustratingly,yang2015unsupervised}. The key idea is to learn to distill the domain-invariant properties from explicitly defined features, such as word n-grams. However, this idea is not directly applicable to deep learning methods because the learned mapping from inputs to representations lacks interpretability in this case.

Recently, there has been an increasing amount of deep learning work on domain adaptation for NLP tasks. A number of earlier researches propose to train an autoencoder on both domains \cite{glorot2011domain,chen2012marginalized,chopra2013dlid}. Later, \newcite{zhou2016bi} proposes to minimize the distribution shift over domains in a linear data combination manner. Other methods on inducing abstract transferable representations include transduction learning \cite{sener2016learning} and residual transfer networks \cite{long2016unsupervised}. In contrast, we use adversarial training to encourage learning domain-invariant features in a more explicit way. Our approach also offers another two advantages over prior work. First, we jointly optimize features with the final classification task while previous work only learns task-independent features using autoencoders. Second, our model can handle classification regarding a particular aspect in texts, while previous methods only operate on an overall representation of an input.

Our approach closely relates to the idea of domain-adversarial training. Adversarial networks have originally been developed for image generation \cite{goodfellow2014generative,makhzani2015adversarial}, and later applied to domain adaption in computer vision \cite{ganin2014unsupervised,ganin2015domain,domain_separation_nets16} and speech recognition \cite{shinohara2016adversarial}. While \newcite{ganin2015domain} also apply this idea to sentiment analysis, their practical gains have remained limited. We departure from this work from at least two aspects: 1) our model is aspect-augmented and 2) we provide detailed analysis and achieve a more robust adversarial training through the use of reconstruction loss. As our experiments demonstrate these advancements result in improved performance.


\paragraph{Aspect-based Text Classification} Our aspect-augmented model also relates to previous work on rationale/aspect-based classification \cite{zaidan2007using,marshall2015robotreviewer,zhang2016rationale,brun-perez-roux:2016:SemEval}. These methods typically rely on human-provided rationales to improve prediction. In contrast, our model only assumes access to a small set of keywords as a source of weak supervision. Attention-based models, on the other hand, offer an unsupervised mechanism to induce \emph{soft} attention over each unit in texts \cite{bahdanau2014neural,rush2015neural,chen2015abc,cheng2016long,xu2015show,xu2015ask,yang2015stacked,martins2016softmax}. However, such attention is learned with a large amount of labeled data while our work assumes no annotations in the target domain. Most recently, \newcite{lei2016rationalizing} introduce a stochastic attention mechanism that selects \emph{hard} rationales in an unsupervised manner. However, similarly
to attention models, this rationale selections is also learned using labeled data. Moreover, all prior approaches focus on in-domain classification. In this paper, however, we study aspect-based classification in the context of domain adaptation. 

% Domain-Adversarial Training of Neural Networks
% Adversarial Multi-Task Learning of Deep Neural Networks for Robust Speech Recognition
% Revisiting Batch Normalization For Practical Domain Adaptation
% Bi-Transferring Deep Neural Networks for Domain Adaptation, a linear data reconstruction manner
% Deep learning for domain adaptation by interpolating between domains
%Deep Learning for Aspect-Based Sentiment Analysis, assume gold relevance score. 1
% brun-perez-roux:2016:SemEval
% Show, attend and tell: Neural image caption generation with visual attention
% Rationale-Augmented Convolutional Neural Networks for Text Classification



==> old-results.tex <==
%\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
%\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut

\begin{table*}[t]
    \centering
    \begin{tabular}{llcccccc}
	\toprule
	%\hline
	\multicolumn{2}{c}{\textsc{Domain}} & \multirow{2}{*}{~~~SVM~~~} & \multirow{2}{*}{~~~mSDA~~~} & ~Source~ & \multirow{2}{*}{~Ours-NA} & \multirow{2}{*}{Ours-Full} & \multirow{2}{*}{In-Domain}\\
    \textsc{Source} & \textsc{Target} & & & Only & & \\
    \midrule
    Value & \multirow{5}{*}{\begin{tabular}[x]{@{}c@{}}Restaurant\\Overall\end{tabular}} & 82.2 & 84.7 & 87.4 & 89.9 & \tb{90.7} & \multirow{5}{*}{93.4} \\
    Room &  & 75.6 & 80.3 & 79.3 & 80.3 & \tb{88.0} &  \\
    Checkin &  & 77.8 & 81.0 & 83.0 & 80.7 & \tb{85.9} & \\
    Service &  & 82.2 & 83.8 & 88.0 & 88.9 & \tb{89.1} &  \\
    Cleanliness &  & 77.9 & 78.4 & \tb{83.2} & 79.7 & 81.8 &  \\
    \midrule
    \midrule
    %\hline
    \multicolumn{2}{c}{\textsc{Average}}  & 79.1 & 81.6 & 84.2 & 83.9 & \tb{87.1} & 93.4 \\
	\bottomrule
    %\hline
    \end{tabular}
    \caption{\tb{Review:} Classification accuracy (\%) of different approaches on the reviews dataset. The hotel reviews from TripAdvisor (source domain) consist of five different aspects while the restaurant reviews from Yelp (target domain) has labels only for a single \emph{overall} aspect. Boldface numbers indicate the best accuracy for each testing scenario.}\label{tb:review}
\end{table*}

\section{Results}\label{sec:result}

In this section, we first show the main comparisons of the prediction accuracy between our model and other baselines. In Section \ref{sec:analysis}, we provide a more detailed analysis on each component of our model and demonstrate their impact to the model performance.

\subsection{Main Results}\label{sec:main}

Table \ref{tb:pathology} summarizes the classification accuracy of different methods on the pathology dataset, including the results of six domain adaptation tasks. Our full model (Ours-Full) consistently achieves the best performance on each task compared to other baselines and model variations. It is not surprising that SVM and mSDA perform poorly on this dataset because they only predict labels based  on an overall feature representation of the input. Thus they are unable to predict labels for a particular aspect in the report. Compared to Ours-NA, our model achieves a significant improvement of 22.5\% (94.2\% vs 71.7\%) on average. Note that Ours-NA uses the same set of labeled and unlabeled data as our model, and the only difference is that Ours-NA has no adversarial training. As a reference, we also provide a performance upper bound by training our model on the full labeled set in the target domain, denoted as In-Domain in the last column of Table \ref{tb:pathology}. On average, the accuracy of our model is only 2.6\% behind this upper bound.

Table \ref{tb:review} shows the results of domain adaptation from each aspect in the hotel reviews to the overall ratings of restaurant reviews. Our full model achieves the best performance on four out of five adaptation tasks. On average, our full model outperforms Ours-NA by 3.2\% (87.1\% vs. 83.9\%). The gains are more prominent when using room quality and checkin service aspects as the source domain, reaching 7.7\% and 5.2\%, respectively. The last column shows the in-domain supervised accuracy (93.4\%) using 100k restaurant reviews. 

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figures/recon_heat.pdf}
%\vspace{-0.11in}
\caption{Heat map of $150\times 150$ matrices. Each row corresponds to the vector representation of a document that comes from either the source domain (top half) or the target domain (bottom half). The left matrix is generated by our model without the reconstruction loss function and the right one is generated by our full model.}\label{fig:heat}
\end{figure}


\subsection{Analysis}\label{sec:analysis}

\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{figures/neighbor.pdf}
\caption{Examples of restaurant reviews and their nearest neighboring hotel reviews induced by different models (column 2 and 3). The distance between reviews is measure by the cosine similarity between their vector representations induced by the model. For hotel reviews, the room quality is the focal aspect and we show the sentences that have high relevance score. The sentiment phrases of each review are in blue, and some reviews are also shortened for space.}
\label{fig:neighbor}
\end{figure*}

\begin{table}[t]
    \centering
    \begin{tabular}{lcccc}
	\toprule
    \multirow{2}{*}{\textsc{Dataset}} & \multicolumn{2}{c}{Ours-Full} &  \multicolumn{2}{c}{Ours-NA}\\
    \cmidrule(lr){2-3} \cmidrule(l){4-5}
     & -REC. & +REC. & -REC. & +REC.\\
    \midrule
    \textsc{Pathology} & 90.4 & 94.2 & 68.8 & 71.7 \\
    \textsc{Review} & 80.4 & 87.1 & 85.4 & 83.9 \\
    \bottomrule
    \end{tabular}
    \caption{Impact of adding the reconstruction component in the model, measured by the average accuracy on each dataset. +REC. and -REC. denote the presence and absence of the reconstruction loss, respectively. }\label{tb:recon}
\end{table}

\paragraph{Impact of the reconstruction loss} We first analyze the impact of adding embedding reconstruction loss in the learning objective. Figure \ref{fig:heat} shows the heat maps of the learned document representations from either the source domain (top half) or the target domain (bottom half) on the review dataset when room quality is the focal aspect. There is no significant distribution difference between the top and the bottom half of the matrices, indicating domain-invariance of learned representations in both cases. However, the left matrix (w/o reconstruction) is much more sparse than the right one (with reconstruction). Almost 85\% entries of the left matrix have small values ($<10^{-6}$) while the sparsity is only about 30\% for the right one. Moreover, the standard deviation of the right matrix is also ten times higher than the left one. These comparisons demonstrate that the reconstruction loss function improves both the richness and diversity of the learned representations. 

Table \ref{tb:recon} summarizes the impact of the reconstruction loss on model performance. For our full model (Ours-Full), adding the reconstruction loss yields an average of 3.8\% gain on the pathology dataset and 6.7\% on the review dataset. However, in the case of no adversarial training (Ours-NA), adding the reconstruction component has no clear effect. This is expected because the main motivation of adding this component is to achieve a more robust adversarial training.

\begin{table}[t]
    \centering
    \begin{tabular}{lcc}
	\toprule
     & \textsc{Pathology} & \textsc{Review} \\
     \midrule
     w/o Relevance Score & 69.5 & 87.0 \\
     w/ Relevance Score & 94.2 & 87.1 \\
    \bottomrule
    \end{tabular}
    \caption{Comparisons of average accuracy on each dataset if removing the relevance scoring component from the model. }\label{tb:relevance}
\end{table}

\paragraph{Impact of relevance scoring} Next we analyze the impact of the aspect-relevance scorer on model performance. As shown in Table \ref{tb:relevance}, the relevance scoring component has more significant impact on the pathology reports dataset (+24.7\%) than on the review dataset (+0.1\%). This is because on the pathology dataset our task is to adapt the model from one aspect to another within the \emph{same} set of reports. Therefore, it is essential for the model to have the capacity of distinguishing between different aspects in this case. In contrast, on the review dataset, different aspects in hotel reviews are highly correlated, and their labels are often consistent to each other.

\begin{table}[t]
    \centering
    \begin{tabular}{lccc}
	\toprule
    \textsc{Dataset} & $\lambda^t=0$ & $0<\lambda^t<\infty$ & $\lambda^t=\infty$ \\
    \midrule
    \textsc{Pathology} & 86.9 & 94.2 & 79.0 \\
    \textsc{Review} & 80.1 & 87.1 & 85.7 \\
    \bottomrule
    \end{tabular}
    \caption{The effect of regularization of the transformation layer on the performance. $\lambda^t=0$ indicates no regularization on transformation and $0<\lambda^t<\infty$ corresponds to our model. $\lambda^t=\infty$ corresponds to the removal of the transformation layer because the transformation is always identity in this case. }\label{tb:transformation}
\end{table}


\paragraph{Regularization on the transformation layer} Table \ref{tb:transformation} shows the model accuracy with different regularization weights $\lambda^{t}$ in Equation \ref{eq:transformation}. We change  $\lambda^{t}$ to reflect different model variations. First, our model performs better than $\lambda^{t}=\infty$ on both datasets, indicating the importance of adding the transformation layer. Second, no regularization $\lambda^{t}=0$ also consistently results in inferior performance. Actually, we note that the results of $\lambda^{t}=0$ are close to the accuracy of our model without the reconstruction loss, as shown in the first column of Table \ref{tb:recon}. This is not a coincidence because a transformation without regularization has too much flexibility and will dilute the effect from reconstruction. As a result, the adversarial training will fail in a similar way to the case of no reconstruction loss.

\paragraph{Examples of neighboring reviews} Finally, we illustrate in Figure \ref{fig:neighbor} a case study on the properties of learned document representations by different models. The first column shows two example restaurant reviews that have similar representations by either Ours-Full or Ours-NA. Sentiment phrases in these examples are in blue color and are mostly food-specific, such as ``undercooked'' and ``closer to bland''. In the other two columns, we show example hotel reviews that are nearest neighbors to the restaurant reviews, measured by cosine similarity between their representations. In column 2, many sentiment phrases are specific for room quality, such as ``old'' and ``rained water from above''. Our full model successfully learns to eliminate domain-specific information and to map those domain-specific words into similar domain-invariant representations. In column 3, however, most sentiment phrases are common (e.g. old) or about food (e.g. food poison). This demonstrates that Ours-NA only captures domain-invariant features from phrases that commonly present in both domains. 

\com{
\begin{table}[t]
    \centering
    \begin{tabular}{lcccc}
	\toprule
    \textsc{~Method~} & \textsc{Syn1} & \textsc{Syn2} & \textsc{Syn3} & \textsc{Syn4} \\
    \midrule
    ~Ours-NA & 75.4 & 52.8 & 100.0 & 49.2 \\
    ~Ours-Full & 99.8 & 100.0 & 100.0 & 100.0 \\
    \bottomrule
    \end{tabular}
    \caption{Classification accuracy on four synthetic datasets that represent different challenges in domain adaptation.}\label{tb:synthetic}
\end{table}

\paragraph{When adversarial training is useful?} As shown in Table \ref{tb:pathology} and \ref{tb:review}, the gains from using adversarial training vary significantly over different adaptation scenarios. To better understand when adversarial training is useful, we further test on four synthetic datasets that represent different challenges in domain adaptation. Specifically, each synthetic document consists of several randomly generated sentences. Each sentence is always associated with a random aspect and contains a special token as the aspect name (e.g. \texttt{ASPECT0\_NAME0}) and another special token as the aspect polarity (e.g. \texttt{ASPECT0\_POSITIVE0}).\footnote{Aspects, names and polarity tokens each have about ten options.} Document labels are either positive or negative, indicated by the polarity tokens of the focal aspect, except for the first dataset (see below). The adaptation task is to transfer the model from one aspect to another. The characteristics of each dataset are as follows.

\begin{itemize}[leftmargin=12pt,parsep=-2pt,topsep=2pt]
\item \textsc{Syn1:} Positive if the name of the focal aspect  (e.g. \texttt{ASP0\_NAME0}) occurs, otherwise negative. 

\item \textsc{Syn2:} Positive polarity tokens have 20\% overlap across domains (the focal aspects). Negative polarity tokens have no overlap.

\item \textsc{Syn3:} Both positive and negative polarity tokens have 20\% overlap across domains.

\item \textsc{Syn4:} Both positive and negative polarity tokens have 5\% overlap across domains.
\end{itemize}
Table \ref{tb:synthetic}
}



==> old-setup.tex <==
\begin{figure*}[t]
\vspace{-0.1in}
\centering
\includegraphics[width=0.95\textwidth]{figures/model_new.pdf}
%\vspace{-0.11in}
\caption{Aspect-augmented adversarial network for domain adaptation. The model is composed of (a) an aspect-driven document encoder, (b) a label predictor and (c) a domain classifier.
%Each document is encoded in a relevance weighted, aspect-dependent manner and passed on to both the primary label classifier and the domain classifier as the adversary to ensure invariance. Parameters of all the components are learned jointly during training.
}
\label{fig:model}
\end{figure*}

\section{Experimental Setup}\label{sec:setup}

\begin{table}[t]
\begin{small}
    \centering
    \begin{tabular}{llcc}
	\toprule
    \multicolumn{2}{l}{\textsc{Dataset}} & \#Labeled & \#Unlabeled \\
    \midrule
    \multirow{4}{*}{\textsc{Pathology}} & DCIS & 23.8k & \multirow{4}{*}{96.6k} \\
     & LCIS & 10.7k &  \\
     & IDC & 22.9k &  \\
     & ALH & 9.2k &  \\
     \midrule
    \multirow{2}{*}{\textsc{Review}} & Hotel & 100k & 100k \\
     & Restaurant & - & 200k \\
    \bottomrule
    \end{tabular}
\end{small}
    \caption{Statistics of the pathology reports dataset and the reviews dataset that we use for training. The same set of unlabeled reports is used for all different aspects in the pathology reports dataset.}\label{tb:data}
\end{table}


\paragraph{Pathology dataset} 
We first use the breast pathology reports dataset that are collected from three partner hospitals. This dataset contains a total of 96.6 thousand pathology reports. The pathology reports typically include diagnosis results for more than 20 different aspects that are related to breast cancer disease. In our experiments, we focus on four aspects: Ductal Carcinoma In-Situ (DCIS), Lobular Carcinoma In-Situ (LCIS), Invasive Ductal Carcinoma (IDC) and Atypical Lobular Hyperplasia (ALH). 

We explore the domain adaptation problem from one aspect to the other. For example, we want to train a model on annotations of DCIS and apply it on LCIS. Each aspect has two possible class labels, positive or negative. For annotations, we use the combination of the data used in \cite{buckley2012feasibility} and the data from Breast Cancer Database (BCD). Table \ref{tb:data} summarizes the statistics of labeled data for each aspect. We use a held out of 500 reports as the development set (source domain) or the testing set (target domain). We also use the common names of each aspect as a source of weak supervision for learning the relevance scorer. On average, each aspect has about two to three different name variations and they can be easily provided by a doctor. 
%All reports were automatically anonymized for privacy, and we further use NLTK 3.0 for sentence split and tokenization. 


\paragraph{Review dataset}
For our second application, we use a review dataset. As the source domain, we use the hotel reviews dataset that is used in previous work \cite{wang2010latent,wang2011latent}. For the target domain, we use the restaurant reviews dataset from Yelp.\footnote{\url{https://www.yelp.com/dataset_challenge}} Both datasets have ratings on a scale of 1 to 5 stars. We label reviews with ratings $>3$ as positive and those with ratings $<3$ as negative, and we discard the rest. The hotel dataset includes a total of around 200k reviews collected from TripAdvisor,\footnote{\url{https://www.tripadvisor.com/}} so we split 100k as labeled and the other 100k as unlabeled data. We randomly select 200k restaurant reviews as the unlabeled data in the target domain. We use a held out of 2k reports as the development set (source domain) or the testing set (target domain). Table \ref{tb:data} summarizes the statistics of the review dataset.

The hotel reviews naturally have ratings for six aspects, including \emph{value}, \emph{rooms} quality, \emph{checkin} service, room \emph{service}, \emph{cleanliness} and \emph{location}. We use the first five aspects because the sixth aspect \emph{location} has positive values for over 95\% of the reviews and thus the trained model will suffer from the lack of negative examples. The restaurant reviews, however, only have single ratings for an \emph{overall} impression. Therefore, we explore the task of adaptation  from each of the five hotel aspects to the restaurant domain. The hotel reviews dataset also provides a total of 290 keywords for different aspects that are generated by the bootstrapping method used in \cite{wang2010latent}. We use those keywords as supervision for learning the relevance scorer.

\begin{table}[t]
    \centering
    \begin{tabular}{@{~}lc@{~~~}cc@{~~~}c@{~}}
	\toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c}{Source} & \multicolumn{2}{c}{Target} \\
    \cmidrule(lr){2-3} \cmidrule(l){4-5}
     & Label & Unlabel & Label & Unlabel \\
    \midrule
    SVM & \Yes & \No & \No & \No \\
    mSDA & \Yes & \Yes & \No & \Yes \\
    SourceOnly & \Yes & \Yes & \No & \No \\
    Ours-NA & \Yes & \Yes & \No & \Yes \\
    Ours-Full & \Yes & \Yes & \No & \Yes \\
    In-Domain & \No & \No & \Yes & \No \\
    \bottomrule
    \end{tabular}
    \caption{Usage of labeled and unlabeled data in each domain by our model and other baseline methods. }\label{tb:usage}
\end{table}


\begin{table*}[t]
    \centering
    \begin{tabular}{llcccccc}
	\toprule
	%\hline
	\multicolumn{2}{c}{\textsc{Domain}} & \multirow{2}{*}{~~~SVM~~~} & \multirow{2}{*}{~~~mSDA~~~} & ~Source~ & \multirow{2}{*}{~Ours-NA} & \multirow{2}{*}{Ours-Full} & \multirow{2}{*}{In-Domain}\\
    \textsc{~Source} & \textsc{Target~} & & & Only & & \\
	\midrule
    %\hline
    ~IDC & ALH & 64.4 & 65.4 & 66.4 & 52.6 & \tb{93.8} & 96.8 \\
    ~ALH & IDC & 37.0 & 36.2 & 26.8 & 27.6 & \tb{92.0} & 96.8 \\
    \midrule
    %\hline
    ~DCIS & IDC & 94.0 & 94.0 & 77.4 & 92.4 & \tb{94.6} & 96.8 \\
    ~IDC & DCIS & 71.8 & 73.0 & 62.4 & 87.6 & \tb{95.0} & 96.2\\
    \midrule
    ~LCIS & DCIS & 45.8 & 45.0 & 25.2 & 81.2 & \tb{93.8} & 96.2 \\
    ~DCIS & LCIS & 73.8 & 76.2 & 75.4 & 89.0 & \tb{96.0} & 97.8 \\
    \midrule
    \midrule
    %\hline
    \multicolumn{2}{c}{\textsc{Average}}  & 64.5 & 65.0 & 55.6 & 71.7 & \tb{94.2} & 96.8 \\
	\bottomrule
    %\hline
    \end{tabular}
    \caption{\tb{Pathology:} Classification accuracy (\%) of different approaches on the pathology reports dataset, including the results of six adaptation scenarios from four different aspects (IDC, ALH, DCIS and LCIS) in breast cancer pathology reports. ``mSDA'' indicates the marginalized denoising autoencoder in \protect\cite{chen2012marginalized} and ``Ours-NA'' corresponds to our model without the adversarial training component. We also include in the last column the in-domain supervised training results of our model as the performance upper bound. Boldface numbers indicate the best accuracy for each testing scenario.}\label{tb:pathology}
\end{table*}

\paragraph{Baselines} We compare against different baselines and variants of our model
% Ours-NA, SVM, mSDA, Source Only, data usage table
\begin{itemize}[leftmargin=10pt,parsep=-4pt,topsep=0pt]

\item \textbf{SVM}: the linear SVM baseline trained on the raw bag-of-words representation of labeled data on source and test it on target.

\item \textbf{mSDA}: marginalized Stacked Denoising Autoencoders \cite{chen2012marginalized}, a domain adaptation algorithm that outperforms both prior deep learning and shallow learning approaches.\footnote{We use the publicly available implementation provided by the authors at \url{http://www.cse.wustl.edu/~mchen/code/mSDA.tar}}

\item \textbf{SourceOnly}: our model trained with only labeled and unlabeled data in the source domain. No target domain data is used.

\item \textbf{Ours-NA}: our model without the adversarial component. To implement this model we simply set the strength of adversarial training to zero.

%\item \textbf{In-Domain}: supervised model trained on in-domain annotation as the performance upper bound.

\end{itemize}
Table \ref{tb:usage} summarizes the usage of labeled and unlabeled data in each domain by our model and different baselines. Note that our model assumes the same set of data as Ours-NA and mSDA methods.


\paragraph{Implementation details}
Following prior work \cite{ganin2014unsupervised}, we gradually increase the adversarial strength $\rho$ and decay the learning rate during training. We also apply batch normalization \cite{ioffe2015batch} on the sentence encoder and dropout with ratio 0.2 on word embeddings and each hidden layer activation. We set the hidden layer size to 150 and pick the transformation regularization weight $\lambda^{t}=0.1$ for the pathology dataset and $\lambda^{t}=10.0$ for the review dataset. 
%We use Adam \cite{kingma2015method} as the optimization method with the default setting suggested by the authors. 
